In situ growth of a type-II ZnO/ZnS heterostructure:From stability to band-offset

We have successfully obtained a ZnO/ZnS heterostructure by heating a ZnS(001) single crystal in a controlled impurities-free oxygen atmosphere. Combining X-ray photoelectron spectroscopy (XPS), and atomic force microscopy (AFM), we explore the stability, electronic structure, and morphology of that interface. Our XPS measurements reveal a binding energy shift of the core-level peaks, indicating a band-bending effect due to the formation of a hybrid ZnO/ZnS interface. In addition, AFM measurements show that exposure of ZnS single-crystal to an oxygen atmosphere leads to the formation of ZnO/ZnS-like islands. Interestingly, our band-offset estimation suggest a type-II heterostructure arrangement with suitable electronic edges positions that turn ZnO/ZnS heterostructure a promising platform for catalytic applications, particularly hydrogen and oxygen evolution reactions.

==> FurtherParts/DataAvailability.tex <==
\section*{Data availability}
All relevant data are included in the paper and the Supporting Information.

==> Results/Theoretical/Theoretical.tex <==
\section{Theoretical Results}
\subsection{Point defect stability and electronic structure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=1.0\textwidth]{Results/Theoretical/formation_energy-new-2.pdf}
    \caption{Formation Energy of (a) Zinc and (b) Sulfur vacancy as a function of the electronic chemical potential in an S-rich scenario.}
    \label{fig-Form}
\end{figure}

The formation energy of defect $D$ in a particular charge state $q$ ($E_{form}(D^{q})$) is a well-known strategy for describing the stability of point defects \cite{Janotti2007}. Considering the different charge states ($q= -2,-1, 0, 1, 2$) for zinc and sulfur vacancy in an S-rich scenario we computed the formation energy (See SI) as a function of the electronic chemical potential $\mu_{e}$ as depicted in Fig. \ref{fig-Form}. In the neutral defect picture (i.e, $q = 0$), zinc vacancy is more stable than sulfur vacancy ($E_{form}(V_{Zn}^{0}= 1.3 \ eV)$ , $E_{form}(V_{S}^{0}= 3.9 \ eV)$).  In addition, With $\mu_{e}$ pinned at the top of valence band, we obtained $E_{form}(V_{Zn}^{-1}) = 1.56 \  eV$, $E_{form}(V_{Zn}^{-2}) = 2.04 \ eV$, $E_{form}(V_{S}^{+1}) = 3.54 \ eV$,$E_{form}(V_{S}^{+2}) = 3.20 \ eV$, according to Fig.\Ref{fig3}(a) and Fig.\Ref{fig3}(b), respectively. These findings are well-aligned with the general trend  previously reported \cite{Yao2012}, which shows that charged zinc vacancies are more stable than charged sulfur vacancies. Furthermore, in this same scenario ($\mu_{e}$ pinned at the top of the valence band), the formation energy of charged zinc vacancy, especially the $E_{form}(V_{Zn}^{-1})$, is close to that of neutral zinc defects, which suggests that both nature (neutral and charged) of cation defect are equally stable on ZnS and might coexist. On the other hand, according to our calculations, it is expected that if sulfur vacancies are formed on ZnS, it should stay in the charge state $+2$. Overall, the cation-defect ZnS is the most energetic favorable configuration in our system

 An interesting parameter to investigate the nature of the stability (n-type or p-type) in the $V_{Zn}$-ZnS picture is the transitions $\epsilon(q/q')$ highlighted in Fig. \ref{fig-Form}(a)-(b) by the crossing of each line. This parameter computes the particular $E_{fermi}$ value where a transition from a defect in the charge $q$ to $q'$ takes place \cite{Janotti2007}. Zinc vacancy behaves as an acceptor, thus decreasing in energy as $\mu_e$ increases. According to the formation energy calculations, all the possible transition states -$\epsilon(-2/0)$, $\epsilon(-1/0)$, and $\epsilon(-2/-1)$- occur slightly above the VBM. This finding illustrates that zinc vacancies in an S-rich ZnS scenario behaves as shallow-acceptors and are indeed stable as a p-type configuration.
%\newpage
\subsection{Electronic Structure Analysis}

\begin{figure}[h!]
    \centering
    \includegraphics[width=1.0\textwidth]{Results/Theoretical/DOS_corrected-oficial.pdf}
    \caption{Projected Density of states of (a) pristine, (b) $V_{Zn}^0$,(c) $V_{Zn}^{-1}$, (d) $V_{S}^{0}$ and (e) $V_{S}^{+2}$ doped ZnS.The Fermi level was shifted to $0$ eV for clarity.}
    \label{fig3}
\end{figure}

Fig.\ref{fig3} shows the projected density of states of pristine ZnS and ZnS with vacancies. All the structures were calculated taking into account spin-polarization. The final magnetization is zero though. In this sense, Fig.\ref{fig3} shows spin-up projected density of states of such structures. The calculated band gap of the pristine ZnS is 2.2 eV, which is an underestimated value as expected from calculations through PBE-GGA methodology \cite{Perdew2017}. Regarding the total density of states of each system, we found similar characteristics. Firstly, the Zn 3d states dominate the portion far from the valence band. Conversely, the valence band is primarily composed of S 3p states, while the conduction band is mainly formed by Zn 4p and unfilled S 3p states. The main difference between defect-free and defective ZnS is the appearance of a few states inside the gap, indicated by the black arrow in Fig.\ref{fig3}(b)-(e). For instance, after the formation of zinc vacancy (Fig.\ref{fig3}(b)-(c)) there is a rise of a few states slightly above the Fermi-level. This finding is attributed to the decrease in the coordination number of S atoms due to the removal of zinc species, which promotes new S 3p-like states above the Fermi level, as highlighted by the filled red area in Fig.\ref{fig3}(b)-(c) (middle plot). In addition, the band gap is tailored to $~ 2 \ eV$. Although the aforementioned band gap underestimation through PBE-GGA calculations, this trend might indicate an electronic response improvement due to the formation of cation defects. The slight difference between neutral (Fig.\ref{fig3}(b)) and charged (Fig.\ref{fig3} (c)) cation-doped ZnS is the density of such S 3p-like states arising inside the forbidden zone, which seems higher in the case of charged zinc vacancy. Overall, both structures could explain the
enhancement of the electronic and optical response, as pointed out from XPS and PL experiments. On the other hand, the formation of sulfur vacancy gives rise to a few states slightly below the conduction band minimum, as revealed in Fig.\ref{fig3}(d)-(e). The decrease of the Zn coordination due to the removal of sulfur results in some Zn 4p-like states, highlighted by the filled red area in Fig.\ref{fig3}(d)-(e) (bottom panel). However, we did not observe a band gap reduction in either scenario (neutral or charged sulfur vacancy), indicating sulfur vacancies do not significantly improve the electronic response of the system.  This finding might be addressed to the doping concentration limit. In general, sulfur vacancies in zinc blende ZnS are predicted to play a role in electronic and optical properties only at high defect concentration (higher than $25 \%$) \cite{Liu2020}. As mentioned in the methodology, we maintained the doping below 5 $\%$, making sulfur vacancy unlikely to explain our experimental findings. Based on our theoretical calculations, only neutral and charged zinc vacancy align well with the experimental results, particularly regarding the enhancement of the electronic and optical response and the p-type nature of the system. Therefore, we next focus exclusively on these structures to evaluate the optical properties of doped ZnS from a theoretical perspective.

% Optical properties calculation start here

\subsection{Optical properties calculations}

\begin{figure}[h!]
    \centering
    \includegraphics[width=1.0\textwidth]{Results/Theoretical/Absorption_paper2_oficial.pdf}
    \caption{ Theoretical absorption spectra of of (a) pristine, (b) neutral $V_{Zn}$  and (c) charged $V_{Zn}$  ZnS
}
    \label{fig4}
\end{figure}

A broad optical absorption range is a key prerequisite for a material to be considered a potential candidate for photocatalysis and optoelectronic devices applications, as in the case of ZnS. In this sense, Fig.\ref{fig4} compares the optical absorption of ZnS in three particular scenarios: pristine, neutral p-doped, and charged p-doped ZnS. In the first case, the only observed peak was the absorption edge at $3.6$ eV, as shown in Fig.\ref{fig4}(a). This peak corresponds to incident photons with energies matching the ZnS band gap. This result is in good agreement with the experimental band gap of ZnS, as expected, given that all the optical property calculations were performed using $PBE \ -\alpha $  hybrid-functional, with  $\alpha = 0.27$ chosen to fit the experimental band gap value. Conversely, due to the removal of a Zn atom from the pristine ZnS structure, several new absorption peaks were observed. In Fig.\ref{fig4}(b), high absorption peaks at $0.8$ eV (infrared region (IR)), $3.2$ eV, and $3.6$ eV (both in the ultraviolet (UV) range) are shown. The higher intensity of these components indicates that the neutral p-doped ZnS could readily absorb photons with such energies. In addition, the lower intensity absorption peaks are of particular interest, especially the component at $1.8$ eV, corresponding to visible range absorption. This result can be addressed to the formation of a p-type ZnS, highlighting the role of zinc vacancies in enhancing the optical absorption. This improvement was experimentally observed through the green-like emission upon excitation with a $405$ nm laser source, as shown in Fig.\ref{fig2}(b). It is worth noting that before emission, the sample must absorb the incoming photons from the laser source. This step requires an absorption level close to $3.06$ eV. Thus, in view of the new absorption peak at $3.2$ eV in the $V_{Zn}^{0}$-ZnS, this experimental finding might be attributed to the formation of neutral zinc vacancies. On the other hand, in the sight of PL experiment, the neutral zinc defect does not match the results. Once PL  first implies the absorption of photons with a particular source energy, a state at $2.54$ eV in the absorption spectra is required in our experiments. However, changing the charge state of the system to $q=-1$, rather than new components observed in the neutral scenario, a component at $2.7$ eV is found as revealed in Fig.\ref{fig4}(c), in good agreement with the experimental prerequisite. The charged p-type ZnS also displays absorption peaks in a broad range, from IR ($0.7$ eV, $1.08$ eV), visible (VIS) ($1.8$ eV, $2.2$ eV, and $2.7$ eV), and UV interval ($3.6$ eV and $3.8$ eV). It should be noted in the dipole approximation we evaluate the imaginary part of the dielectric function computing direct inter-band transitions by a summation over several empty states, neglecting any many-body effects. Therefore, slight energy differences can occur, as well as a loss of information, as widely discussed \cite{Li2015,Webster2015}. However, all signatures from this model should be retained through an improved methodology, which allows us to attest the good agreement between the experiments and first-principle calculations.


\begin{figure}[h!]
    \centering
    \includegraphics[width=1.0\textwidth]{Results/Theoretical/JDOS_modified.pdf}
    \caption{Joint Density of states (JDOS) of (a) pristine, (b) neutral $V_{Zn}$  and (c) charged $V_{Zn}$  ZnS. Pictorial diagram level illustrating the emissions in the (d) pristine and (e) p-doped scenarios.}
    \label{fig5}
\end{figure}

To address the new PL peaks, a suitable approach is to evaluate the joint density of states (JDOS), which represents the allowed inter-band transitions at specific energy levels. Essentially, it can be understood as an emission-like spectrum, enabling the correlation of defect-induced states with experimental photoluminescence features. Fig.\ref{fig5}(a)-(c) display the JDOS for both pristine and doped ZnS. Our analysis is confined to an energy range that includes IR, VIS, and UV-VIS regions. In the pristine system, there is only one emission, corresponding to a direct recombination process from the VBM to the CBM producing photons with $3.6$ eV. On the other hand, as we previously discussed, density of states (DOS) calculations show that when a p-type structure forms, new states slightly above the VBM emerge. These states can act as trapping sites, enabling recombination processes beyond the direct VBM-CBM transition. \cite{Zott1997}
To clarify the role of shallow levels in the emission spectra of ZnS, Fig. \ref{fig5}(b) to Fig.\ref{fig5}(c) show the JDOS of p-type ZnS, obtained by removing one zinc atom from the pristine supercell. In Fig.\ref{fig5}(b), the neutral configuration is evaluated, revealing new emission lines at $0.8$ eV, $1.5$ eV, and $1.8$ eV, in addition to the $3.6$ eV emission line. The high JDOS peaks at $1.5$ eV and $1.8$ eV suggest a higher probability of these emissions occurring. Therefore, we can infer that zinc vacancies not only enhance optical absorption but also improve optical emission. However, taking PL experiments as the reference, the neutral scenario alone cannot fully explain the two new emissions in the visible range, as discussed in the last section. Thus, we turn our attention to the charged system, depicted in Fig.\ref{fig5}(c). 

The features in this case are quite similar to those in the neutral structure, except for the energy of the emissions. The lowest probability of emission occurs at $1.2$ eV, while the highest JDOS components, apart from the $3.6$ eV peak, fall exactly in the visible range at $1.9$ eV (C I) and $2.2$ eV (C II). This finding aligns well with PL experiments, which revealed two new peaks at $2.05$ eV and $2.12$ eV. Therefore, our ab initio calculations confirm zinc vacancies broadening the ZnS emission lines and suggest these vacancies might be charged in the system. Indeed, as discussed in terms of the formation energy, both neutral and charged zinc vacancies are stable in zb-ZnS and may coexist. The pictorial model distinguishing the pristine and doped scenario is illustrated in Fig.\ref{fig5}(d) to Fig.\ref{fig5}(e). In the pristine scenario (Fig. \ref{fig5}(d), an electron is excited from the valence band to the conduction band. Sequentially, this free excited electron recombines directly into the valence band, emitting a photon with energy $E$, which is equal to the band gap of the system. In contrast, in p-type-like structures, the additional shallow levels in the forbidden zone act as trapping sites. In this case, the free electron that jumped from VBM to CBM recombines at the impurity level $E_{s}$, resulting in an emission whose energy $E'$ is the difference of the band gap and shallow level energy.

